Extension of analytic covers by extension of their ramification divisor

This paper deals with extension of analytic covers. We prove topological extension theorems for analytic covers. The main result is an extension theorem which only uses the extension of the ramification divisor. We give also a Thullen-type and a Hartogs-type extensions theorems.

==> comments.tex <==
\ProvidesFile{Ucyril.fd}[WNCyr Font]
\DeclareFontFamily{U}{wncyr}{}
\DeclareFontShape{U}{wncyr}{m}{n}{<-6>wncyr5<6-8>wncyr7<8->wncyr10}{}
\ProcessOptions

\font\cyr  wncyr10 at 12pt
\font\cyrsm  wncyr10 at 9pt
%\font\cyrb wncyb10 at 12pt

%% wncyr special characters:
%% http://home.vrweb.de/~was/x/pmcyr.pdf
%% E0 and e0   for "e (yo (-mayo))
%% i0 and I0   for j 
%% i1 and I1   for ukr/starorussk. i s tochkoj 
%% N0          for No ("nomer")
%% Kh/kh ili H/h  for "x"  ("xiter")
%% Ts/ts ili C/c  for "tse"
%% Ch/ch ili Q/q  for "che"
%% X/x ili Sh/sh   for "sha"
%% W/w ili shch   for "scha"
%% Ya/ya ili J1/j1  for "ya"
%% Yu/yu ili J2/j2  for "yu"       


%% Vkliuchit' rus : \cyr ili \cyrb ili \cyrsm (cyrillic-small)
%% Nazad : \rm ili \bf ili \sl itd.


%% Remarki na polyax
%for margin notes
{\catcode`\@=11
\gdef\n@te#1#2{\leavevmode\vadjust{%
 {\setbox\z@\hbox to\z@{\strut#1}%
  \setbox\z@\hbox{\raise\dp\strutbox\box\z@}\ht\z@=\z@\dp\z@=\z@%
  #2\box\z@}}}
\gdef\leftnote#1{\n@te{\hss#1\quad}{}}
\gdef\rightnote#1{\n@te{\;\kern-\leftskip#1\hss}{\moveright\hsize}}
\gdef\?{\FN@\qumark}
\gdef\qumark{\ifx\next"\DN@"##1"{\leftnote{\rm##1}}\else
 \DN@{\leftnote{\rm??}}\fi{\rm??}\next@}}
%
\def\lnote#1{\leftnote{\vbox{\hsize=2truecm
\baselineskip =11pt \lineskiplimit =1pt
\footnotesize \noindent #1}}}
%
\def\rnote#1{\rightnote{\vbox{\hsize=1.5truecm
\lineskip =11pt \lineskiplimit =1pt
\tiny \noindent #1}}}
%
%
%% Kommandy : \lnote{Text} ili \rnote{Text}
%% Ili \lnote{\cyr Text} 
%%
%%


%% Cveta:
%% Available colors:
%% \red, \green, \black, \blue \magent

\usepackage{xcolor}

\definecolor{DarkGreen}{rgb}{0,0.6,0} 
\def\red{\color{red}}
\def\green{\color{DarkGreen}}
\def\blue{\color{blue}}
\def\black{\color{black}}
\definecolor{MyMagenta}{rgb}{0.6,0.0,0.5} 
\def\magent{\color{MyMagenta}}

%\endinput

